Multiple Ways of Working with Users to Develop Physically Assistive Robots

Despite the growth of physically assistive robotics (PAR) research over the last decade, nearly half of PAR user studies do not involve participants with the target disabilities. There are several reasons for this -- recruitment challenges, small sample sizes, and transportation logistics -- all influenced by systemic barriers that people with disabilities face. However, it is well-established that working with end-users results in technology that better addresses their needs and integrates with their lived circumstances. In this paper, we reflect on multiple approaches we have taken to working with people with motor impairments across the design, development, and evaluation of three PAR projects: (a) assistive feeding with a robot arm; (b) assistive teleoperation with a mobile manipulator; and (c) shared control with a robot arm. We discuss these approaches to working with users along three dimensions -- individual vs. community-level insight, logistic burden on end-users vs. researchers, and benefit to researchers vs. community -- and share recommendations for how other PAR researchers can incorporate users into their work.

==> content/textinput-community_researcher.tex <==
\section{The Community Researcher approach}
[Introduction about the idea of community researcher, link to literature, i.e. participatory design]
\subsection{UW Community Researcher}
\subsection{TUDO Community Researcher: Miss L.} [not necessary to keep in here, based on the new structure]
Miss L. has a background in journalism and was diagnosed with Multiple Sclerosis in 1988. She cannot move her arms or legs, is quite shortsighted and sometimes has difficulty speaking out loud. Around 12 years ago, she started getting involved in \ac{HRI} research projects as a community researcher and moved from Berlin to Bremen, Germany. Since then, she has been involved in multiple different \ac{HRI} research projects in varying roles and levels of involvement. The authors of this paper were part of two research projects from 2017 -- 2021 and worked closely together with Miss L. there \cite{arevalo2022does, Pascher.2021recommendations}. 

One of the key benefits we found from working with a community researcher was the reduction of novelty bias and technology fear often associated with robotics research. Miss L., also due to her long lasting experience from working in such projects, was able to interact and reflect on a new robot or interaction technique quite neutrally. Further, she could contrast her experiences with prior usage of other systems, which helped to put novel approaches into context, at least informally.

Miss L.'s presence also helped to bridge the social distance between the researchers and the target user group. For new researchers, it can be challenging to become comfortable with this type of research and know how to approach users from the target group. However, having Miss L. as a community researcher reduced this barrier and made it easier for the team to dive in and understand the specific needs and wants of the users. 

Moreover, Miss L. served as a \enquote{living persona} for the research team. Designing for a specific person, rather than generalizing user needs, helped to overcome the bias often seen in computer science students who tend to overvalue their own needs and priorities. Having a community researcher like Miss L. helped to reduce this bias and ensured that the research was more user-centered.

Additionally, Miss L. provided surprising perspectives that challenged the assumptions of the research team. For example, she made us realize that having a human caregiver around can also be stressful, as it requires constant interaction and may involve dealing with mood swings. This insight highlighted the potential advantage of using a robotic arm to provide independence and support when needed.

Another important contribution of Miss L. was her understanding of the level of adaptability needed for interaction concepts. Due to the wide variability in the remaining motor abilities of users, there is no "one size fits all" technology solution. Miss L's insights shed light on the challenges faced by individuals with different abilities. For example, speech input may work on one day but not on the next due to situational reduction in the ability to speak out loud enough for the system to comprehend. Similarly, head-mounted devices or head-movement-based interactions need to be individually calibrated to accommodate varying levels of mobility.

Furthermore, Miss L. functioned as a pilot participant, not only for robot interaction but also for understanding user needs and fine-tuning the research methodology. Her involvement helped the team to gain practical insights and make necessary adjustments to improve the overall research process.

It is important to note that while working with a community researcher like Miss L. has its advantages, it also requires reflection and balance. There is a need to avoid overvaluing certain needs of the individual and ensure that the research remains objective. However, the overall increase in empathy within the research team and the understanding of the potential impact of the research beyond scientific research papers make the inclusion of a community researcher a valuable asset.

In conclusion, the collaboration with a community researcher like Miss L. proved to be highly beneficial in the development and evaluation of physically assistive robots. Her expertise, personal experiences, and unique perspectives enhanced the research process and provided valuable insights for designing user-centered solutions. Working with a community researcher helped to overcome biases, reduce social distance, and highlight the importance of adaptability in interaction concepts. The involvement of a community researcher also served as a reminder to prioritize the needs and priorities of the users, ultimately leading to more impactful and empathetic research outcomes.

==> content/textinput_homedeployment.tex <==
\section{Home Deployment Stretch}

==> content/textinput_trade_fair.tex <==
\section{Exploring new ways to engage with users: the case for a trade fair approach}
[\textbf{To do}: \begin{itemize}
    \item Link/contrast to the other approaches needed for introduction
    \item integrate references and short explanations to the robotic system we actually developed and tested so people can relate to that
    \item include image of the trade fair setup

\end{itemize}
]

The basic idea behind conducting a study at a trade fair was to bring and set up a robot at a place where there is a high chance for the target group to be present anyhow, thereby minimizing any additional effort needed to participate in a study. 

The trade fair study was conducted at a rehabilitation-focused trade fair (REHACARE\footnote{\emph{REHACARE} trade fair. \url{https://www.rehacare.de}, last retrieved \today.}), which proved to be an ideal environment to engage with a diverse group of participants. The researchers set up a booth where they created a stable robot setup, a bit shielded from the trade fair environment but still open to bystanders. Participants were recruited from different sources, including pre-arranged individuals, interested visitors, and individuals approached during the trade fair. The study employed a team with multiple roles, including moderators for the test sessions, interviewers for questionnaires, assistance, and a \enquote{floater}, responsible for supervising the technology and overall procedure. The team also had a recruiter who engaged with bystanders and potential participants. The trade fair study yielded several important findings and lessons learned. 

First, thorough technology preparation was crucial due to the unpredictable nature of a trade fair environment. A typical lab study may be postponed for a few days in case of unforeseen technical difficulties. A trade fair simply keeps on going. Technical communication issues, such as Bluetooth connectivity problems, highlighted the importance of being present early for setup, bringing necessary replacements, and conducting thorough pilot testing to address potential challenges beforehand.

Second, the busy trade fair environment necessitated adaptable schedules. Participants often preferred to participate on the spot, when they were already bypassing the booth, making it essential to have a larger team capable of filling different roles. Clearly defined time slots for participants proved impractical, emphasizing the need for flexibility and accommodating participants' preferences.

Third, the study demonstrated the delicate trade-off between bystander engagement and study control. Allowing bystanders to observe the study increased the likelihood of their participation and enhanced the ecological validity of the setting. However, this approach also posed challenges in terms of privacy, potential distractions, and interruptions. For us, we decided that the benefit of not closing out bystanders completely was bigger compared to the drawbacks. Certain findings would have not occurred in a more controlled environment. For example, when participants got a bit distracted by bystanders and moved their heads toward them, that interfered with their interaction with the robot (we tested a head-based interaction). In this setup, we could therefore see how they were able to recover and adjust their behavior. But it also meant that we were not able to collect quantitative data reliably. For that, a more enclosed setup is necessary, which is more expensive and requires more preparation on a trade fair.  

Finally, the trade fair study revealed the remarkable diversity among participants. The unfiltered nature of engaging with participants at a trade fair resulted in a broader range of individuals compared to previous studies. This diversity provided valuable insights into the needs and preferences of potential end users.


